Belief revision in the propositional closure of a qualitative algebra

Belief revision is an operation that aims at modifying old be-liefs so that they become consistent with new ones. The issue of belief revision has been studied in various formalisms, in particular, in qualitative algebras (QAs) in which the result is a disjunction of belief bases that is not necessarily repre-sentable in a QA. This motivates the study of belief revision in formalisms extending QAs, namely, their propositional clo-sures: in such a closure, the result of belief revision belongs to the formalism. Moreover, this makes it possible to define a contraction operator thanks to the Harper identity. Belief revision in the propositional closure of QAs is studied, an al-gorithm for a family of revision operators is designed, and an open-source implementation is made freely available on the web.

==> algo-rev-PCQA.tex <==
\def\alors{\textbf{then}}
\def\commentaire#1{\strut\hfill\emph{// #1}}
\def\echec{\fm{failure}}
\def\faire{\textbf{do}}
\def\finsi{\textbf{end if}}
\def\finpour{\textbf{end for}}
\def\IND{~~~~} % indentation
\def\pourchaque{\textbf{for each}\xspace}
\def\etchaque{\textbf{and each}\xspace}
\def\return{\textbf{return}\xspace}
\def\si{\textbf{if}\xspace}
\def\sinonsi{\textbf{else if}\xspace}
%
\def\resultat{\fm{result}}
\def\unerevision{\fm{rev}}
%
\begin{figure}
  $\RevisionQACP(\psi, \mu)$
  \begin{description}
  \item[input]
    $\psi, \mu\in\logiqueQACP$
  \item[output]
    $\revision\in\logiqueQACP$ such that $\revision\equiv\psi\revDist\mu$
  \end{description}
  \begin{enumerate}[\small1\normalsize]
  \item
    $\psi\aff\DNFWoN(\psi)$ \hfill$\psi=\bigvee_i\psi_i$ where $\psi_i\in\logiqueQA$
  \item
    $\mu\aff\DNFWoN(\mu)$   \hfill$\mu=\bigvee_j\mu_j$ where $\mu_j\in\logiqueQA$
  \item
    $\resultat\aff\emptyset$
  \item
    $\distmax\aff+\infty$
  \item
    \pourchaque $i$ \etchaque $j$ \faire
  \item
    \IND$\unerevision\aff\RevisionQA(\psi_i, \mu_j, \distmax)$
  \item
    \IND\si $\unerevision\neq\echec$ \alors
  \item
    \IND\IND$(\revision_{ij}, \distPsiMu_{ij})\aff\unerevision$
            \commentaire{$\revision_{ij}=\psi_i\revDist\mu_j\in\logiqueQACP$}\\
            \commentaire{$\distPsiMu_{ij}=\dist(\Mod(\psi_i), \Mod(\mu_j))$}
  \item
    \IND\IND\si $\distPsiMu_{ij}<\distmax$ \alors
  \item
    \IND\IND\IND$\distmax\aff\distPsiMu_{ij}$
  \item
    \IND\IND\IND$\resultat\aff\{\revision_{ij}\}$
  \item
    \IND\IND\sinonsi $\distPsiMu_{ij}=\distmax$ \alors
  \item
    \IND\IND\IND$\resultat\aff\resultat\cup\{\revision_{ij}\}$
  \item
    \IND\IND\finsi
  \item
    \IND\finsi
  \item
    \finpour
  \item
    $\revision\aff\bigvee_{\scenario\in\resultat}\scenario$
  \item
    \return $\revision$
  \end{enumerate}
\caption{Algorithm for $\revDist$ in $(\logiqueQACP, \modelsCP)$.\label{algo:rev-QACP}}
\end{figure}



==> exemple-revision-EDT-generalise.tex <==
\def\nr{---} % nr = non renseigné
\begin{table*}[bt]
\begin{center}
 \begin{tabular}{|c|c|c|c|c|c|c|c|}
 \cline{3-8}
 \multicolumn{2}{c|}{\strut}  & \multicolumn{3}{c|}{\revisorQA} & \multicolumn{3}{c|}{\revisorPCQA} \\
  \hline
 $n$ & $p$ & \#Variables & Avg distance & Avg time (s) & \#Variables & Avg distance & Avg time (s)  \\  \hline
 3   & 0 & 7  & 24.0 & 1.387    & 6  & 22.0 & 3.809    \\  \hline
 3   & 1 & 8  & 21.0 & 5.407    & 6  & 20.0 & 7.744    \\  \hline
 4   & 0 & 9  & 25.3 & 444.927  & 8  & 24.7 & 119.136  \\  \hline
 4   & 1 & 10 & 29.3 & 765.125  & 8  & 29.3 & 183.945  \\  \hline
 4   & 2 & 11 & 14.0 & 2040.551 & 8  & 14.0 & 266.667  \\  \hline
 5   & 0 & 11 & \nr  & \emph{$>$ 1 hour} & 10 & 26.0 & 3052.398 \\  \hline
 5   & 1 & 12 & \nr  & \emph{$>$ 1 hour} & 10 & \nr  & \emph{$>$ 1 hour} \\  \hline
 \end{tabular}
 \end{center}
 \caption{%
   Average distance and average time according to the problem, parametrized
    by $n$ and $p$, where $n$ is the number of courses and of time periods and
    $p$ is the number of breaks during the global time period.
   ``Avg distance'' is the average of the $\distPsiMu$ values on the set of
     revision problems generated for a given pair $(n, p)$.
   \label{tab-time}}
\end{table*}
%             ------------------
\subparagraph{The second example}
%             ------------------
%
 generalizes the first one.
It consists in a family of examples parametrized
 by $n$ and $p$, where $n$ is the number of courses and of
 time periods (the first example corresponds to $n=4$) and 
 $p$ is the number of breaks during the global time period 
 (the first example corresponds to $p=0$).
Moreover, the breaks in the examples are uniformally spread
 throughout the whole period.
It has been experimented with $n\in\{3, 4, 5\}$ and 
$p\in\{0, 1, 2\}$. Following similar formalizations in $\logiqueAllen$
 (with $2n+p+1$ variables) and $\logiqueAllenCP$
 (with $2n$ variables), the result were the same 
 (except for the additional variables)
 and the computing times are presented in table~\ref{tab-time}.
 The average time, for each line, is computed with series of $n-1$ tests with $d>0$, 
 on a computer with a \mes{2.53}{GHz} processor and \mes{8}{GB} of available memory. 
 For example, for $n=4$ and $p=1$, 
 the average distance is $14.0$ for \revisorQA and \revisorPCQA 
 and the average time is \mes{765.125}{s} for \revisorQA and \mes{183.945}{s} for \revisorPCQA. 
 The average time increases with the number of variables for \revisorQA and 
 for \revisorPCQA. For the same number of variables, \revisorQA is faster than 
 \revisorPCQA. However, as fewer additional variables are introduced under 
 \revisorPCQA, more complex problems can be solved with \revisorPCQA than 
 with \revisorQA.


==> exemple-revision-EDT.tex <==
\def\Cours{\fm{Courses}}
\def\Periodes{\fm{Periods}}
%
\def\anglais{\fm{English}}
\def\biologie{\fm{biology}}
\def\histoire{\fm{history}}
\def\mathematiques{\fm{maths}}
%
\def\huitneuf{\fm{8-9}}
\def\neufdix{\fm{9-10}}
\def\dixonze{\fm{10-11}}
\def\onzedouze{\fm{11-12}}
\def\huitdouze{\fm{8-12}}
\def\Zoe{\text{Zo{\'e}}}
%
%             -----------------
\subparagraph{The first example}
%             -----------------
%
 aims at showing that some revision problems are more easily
 expressed in $\logiqueQACP$ than in $\logiqueQA$.
Let us consider $\Zoe$, a school principal that has to schedule a morning with $4$
 courses in biology, English, history and maths for a group of students.
For this purpose, she plans to reuse the previous year schedule:
 \begin{align*}
   \pi
   &=
   \anglais\eqAQ\huitneuf
   \;\land\;
   \biologie\eqAQ\neufdix
   \\
   \;&\land\;
   \histoire\eqAQ\dixonze
   \;\land\;
   \mathematiques\eqAQ\onzedouze
 \end{align*}
 stating, e.g., that the English course takes place from $8$ to $9$ a.m.

She also has some background knowledge that she expresses first
 in $\logiqueAllen$.
She knows the relation between the $4$ time periods:
 \begin{align*}
   \beta_1
   =
   \huitneuf\mAQ\neufdix
   \;\land\;
   \neufdix\mAQ\dixonze
   \;\land\;
   \dixonze\mAQ\onzedouze
 \end{align*}
Then, she states that every course $c_1$ has no intersection
 (except, possibly, on one of the boundaries) with another course $c_2$:
 \begin{align*}
   \beta_2
   &=
   \bigwedge_{c_1, c_2\in\Cours, c_1\neq{}c_2}
   c_1 \mathrel{{\bAQ}\ourel{\biAQ}\ourel{\mAQ}\ourel{\miAQ}} c_2
   \\
   \text{with }
   \Cours
   &=
   \{\biologie, \anglais, \histoire, \mathematiques\}
 \end{align*}
Then, she aims at representing the fact that each course corresponds to
 one of the $4$ time periods.
Since there is no disjunction in $\logiqueAllen$, she uses the following
 trick:
 asserting that each course is either equal or has no intersection
 (except on the boundaries) with any period:
 \begin{align*}
   \beta_3
   &=
   \bigwedge_{c\in\Cours, p\in\Periodes}
   c \mathrel{{\eqAQ}\ourel{\bAQ}\ourel{\biAQ}\ourel{\mAQ}\ourel{\miAQ}} p
   \\
   \text{with }
   \Periodes
   &=
   \{\huitneuf, \neufdix, \dixonze, \onzedouze\}
 \end{align*}
In order to prevent the courses and the periods to exceed the
 boundaries of the morning, the variable $\huitdouze$ is introduced
 and the following knowledge about it is asserted:
 \begin{align*}
   \beta_4
   &=
   \huitneuf\sAQ\huitdouze
   \;\land\;
   \neufdix\dAQ\huitdouze
   \;\land\;
   \dixonze\dAQ\huitdouze \\
   \;&\land\;
   \onzedouze\fAQ\huitdouze
   \;\land\;
   \bigwedge_{c\in\Cours} c \mathrel{{\sAQ}\ourel{\dAQ}\ourel{\fAQ}} \huitdouze
 \end{align*}
Let $\beta{}=\beta_1\land\beta_2\land\beta_3\land\beta_4$.
Then, the knowledge about the previous year is $\psi=\beta{}\land\pi$.
For the current year, a new constraint is that the biology and history
 teachers should not meet (for some reason):
 \begin{align*}
   \gamma
   &=
   \biologie \mathrel{{\bAQ}\ourel{\biAQ}} \histoire
 \end{align*}
Since the background knowledge has not changed, the knowledge about this
 year is $\mu=\beta{}\land\gamma$.
Thus, to propose a new schedule, $\Zoe$ will revise $\psi$ by $\mu$.
If she uses the $\revDist$ revision operator defined above, there are two
 models that consist in switching English with biology or
 history with maths.

Now, $\Zoe$ wants to formalize its knowledge in $\logiqueAllenCP$.
The previous year schedule $\pi$ and the new constraint $\gamma$ for the
 current years are kept.
What changes is the representation of background knowledge:
 $\CP{\beta}=\beta_1\land\CP{\beta_2}\land\CP{\beta_3}$,
 with $\CP{\beta_2}$ expressing the fact that two courses cannot
 occur in the same period of time
 \begin{align*}
   \CP{\beta_2}
   =
   \bigwedge_{c_1, c_2\in\Cours, c_1\neq{}c_2} \lnot(c_1\eqAQ{}c_2)
 \end{align*}
 and $\CP{\beta_3}$ expressing the fact that each course is in one
 of the $4$ periods:
 \begin{align*}
   \CP{\beta_3}
   =
   \bigwedge_{c\in\Cours}\bigvee_{p\in\Periodes} c \eqAQ p
 \end{align*}
The revision of $\CP{\psi}=\CP{\beta}\land\pi$ by
 $\CP{\mu}=\CP{\beta}\land\gamma$ also gives two models,
 corresponding to the two same course exchanges.
(Formally, they are not the same models, since the sets of
 variables are different---there is an additional variable
 in the first formalization: $\huitdouze$.)

Our claim is that the second formalization is simpler than the first
 one, which has required a ``trick''.
Furthermore, \revisorQA requires about $6$ minutes to solve
 this problem (in the first formalization)
 whereas \revisorPCQA only requires about $2$ minutes.


==> voisinage-Allen.tex <==
{
  \def\Al#1{\ensuremath{\relQCNsa{#1}}}
  \begin{tikzpicture}[node distance=8mm]
    \node(b)[]{\Al{b}} ;
    \node(m)[right of=b]{\Al{m}} ;
    \node(o)[right of=m]{\Al{o}} ;
    \node(oD)[right of=o]{} ; % oD : o à droite
    \node(fi)[above of=oD]{\Al{fi}} ;
    \node(fiH)[above of=fi]{} ; % fiH : fi en haut
    \node(s)[below of=oD]{\Al{s}} ;
    \node(sB)[below of=s]{} ; % sB : s en bas
    \node(eq)[right of=oD]{\Al{eq}} ;
    \node(eqD)[right of=eq]{} ; % eqD : eq à droite
    \node(di)[right of=fiH]{\Al{di}} ;
    \node(d)[right of=sB]{\Al{d}} ;
    \node(si)[above of=eqD]{\Al{si}} ;
    \node(f)[below of=eqD]{\Al{f}} ;
    \node(oi)[right of=eqD]{\Al{oi}} ;
    \node(mi)[right of=oi]{\Al{mi}} ;
    \node(bi)[right of=mi]{\Al{bi}} ;
    %
    \draw[-] (b) -- (m) ;
    \draw[-] (m) -- (o) ;
    \draw[-] (o) -- (fi) ;
    \draw[-] (o) -- (s) ;
    \draw[-] (fi) -- (eq) ;
    \draw[-] (s) -- (eq) ;
    \draw[-] (fi) -- (di) ;
    \draw[-] (s) -- (d) ;
    \draw[-] (di) -- (si) ;
    \draw[-] (eq) -- (si) ;
    \draw[-] (d) -- (f) ;
    \draw[-] (eq) -- (f) ;
    \draw[-] (si) -- (oi) ;
    \draw[-] (f) -- (oi) ;
    \draw[-] (oi) -- (mi) ;
    \draw[-] (mi) -- (bi) ;
  \end{tikzpicture}
}

